Entity-Augmented Distributional Semantics for Discourse Relations

Discourse relations bind smaller linguistic elements into coherent texts. However, automatically identifying discourse relations is difficult, because it requires understanding the semantics of the linked sentences. A more subtle challenge is that it is not enough to represent the meaning of each sentence of a discourse relation, because the relation may depend on links between lower-level elements, such as entity mentions. Our solution computes distributional meaning representations by composition up the syntactic parse tree. A key difference from previous work on compositional distributional semantics is that we also compute representations for entity mentions, using a novel downward compositional pass. Discourse relations are predicted not only from the distributional representations of the sentences, but also of their coreferent entity mentions. The resulting system obtains substantial improvements over the previous state-of-the-art in predicting implicit discourse relations in the Penn Discourse Treebank.

==> con.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\section{Conclusion}
Discourse relations are determined by the meaning of their arguments, and progress on discourse parsing therefore requires computing representations of the argument semantics. We present a compositional method for inducing distributional representations not only of discourse arguments, but also of the entities that thread through the discourse. In this approach, semantic composition is applied up the syntactic parse tree to induce the argument-level representation, and then down the parse tree to induce representations of entity spans. Discourse arguments can then be compared in terms of their overall distributional representation, as well as by the representations of coreferent entity mentions. This enables the compositional operators to be learned by backpropagation from discourse annotations. This approach outperforms previous work on classification of implicit discourse relations in the Penn Discourse Treebank. 

